Learning Object State Changes in Videos: An Open-World Perspective

Object State Changes (OSCs) are pivotal for video understanding. While humans can effortlessly generalize OSC understanding from familiar to unknown objects, current approaches are confined to a closed vocabulary. Addressing this gap, we introduce a novel open-world formulation for the video OSC problem. The goal is to temporally localize the three stages of an OSC -- the object's initial state, its transitioning state, and its end state -- whether or not the object has been observed during training. Towards this end, we develop VidOSC, a holistic learning approach that: (1) leverages text and vision-language models for supervisory signals to obviate manually labeling OSC training data, and (2) abstracts fine-grained shared state representations from objects to enhance generalization. Furthermore, we present HowToChange, the first open-world benchmark for video OSC localization, which offers an order of magnitude increase in the label space and annotation volume compared to the best existing benchmark. Experimental results demonstrate the efficacy of our approach, in both traditional closed-world and open-world scenarios.

==> sec/outline.tex <==
\section{Introduction}

[P1. problem statement; OSC definition] 

\noindent [P2. studying OSC is important]

\noindent [P3. limitations of existing works]

Limitations: (1) small-scale setting: 7/44 OSC categories, one object is tied to a fixed action; (2) human-centric: do not account for the scenario where OSCs happen yet human action is not observable in the video; (3) closed world: the model is only capable of identifying state changes of the object observed during training, poor generalization to novel objects.

\noindent [P4. our dataset+approach]

Our contribution statement: (1) dataset (automated process enabled by LLAMA + collect large-scale human annotation); (2) new problem formulation -- open-world; (3) new self-supervised training pipeline (enabled by CLIP); (4) model design: object-conditioned state prediction (temporal modeling, shared state vocabulary, object-centric feature) to address the open-world challenge.

\section{Approach}
\begin{enumerate}
    \item Formulation: (1) object-centric; (2) open-world. 
    \item Self-supervised training framework, use CLIP to pseudo label every frame
    \item Model design: we propose object-conditioned state prediction to address the open-world challenge with three key designs: (1) shared state vocabulary; (2) temporal modeling; (3) object-centric features.
\end{enumerate}

\section{HT-OSC Dataset \KGnote{better name/acronym?}}
pre-process with LLAMA2; compare with previous datasets (a dataset table);
explain how the focus differs from them (object-centric vs human-centric, there are cases where action is not captured in the video; object going through state change as a passive process)

\section{Experiments}
\subsection{Evaluation}
Evaluate on: (1) ChangeIt~\cite{}; (2) ChangeIt (novel object split); (3) HT-OSC. \KGnote{be sure to have a clear statement about why the other datasets we cite about state changes are not applicable here or why we choose only these}

\noindent Setting: (1) seen objects; (2) unseen objects during test

\noindent Baselines: (1) zero-shot video-text embedding approaches (CLIP~\cite{}); (2) self-supervised casual ordering-enabled approaches (LookfortheChange~\cite{}). 
\KGnote{for seen object case, are there not more models from literature we should include for comparisons?}

\subsection{Results}
3 result tables + 1 ablation table 

\subsection{Qualitative Results}
Visualization of the state predictions given by our model and baselines (seen and unseen objects)
